Understanding intermediate layers using linear classifier probes

Neural network models have a reputation for being black boxes. We propose to monitor the features at every layer of a model and measure how suitable they are for classification. We use linear classifiers, which we refer to as "probes", trained entirely independently of the model itself. This helps us better understand the roles and dynamics of the intermediate layers. We demonstrate how this can be used to develop a better intuition about models and to diagnose potential problems. We apply this technique to the popular models Inception v3 and Resnet-50. Among other things, we observe experimentally that the linear separability of features increase monotonically along the depth of the model.

==> paper-linear-classifier-probes.tex <==

% Sharelatex accepts these paths only when we write out the full structure.
% We'll have to do the same thing for figures, unfortunately.

\chapter{Understanding intermediate layers using linear classifier probes}
\label{chap:paper-linear-classifier-probes}

% Works on Sharelatex.
%\renewcommand{\paperroot}{doctorat/document/paper-linear-classifier-probes}

% Works in TeXShop.
\renewcommand{\paperroot}{paper-linear-classifier-probes}


\setcounter{theorem}{0}

\input{\paperroot/introduction}
\input{\paperroot/relatedwork}
\input{\paperroot/probes}
\input{\paperroot/experiments}
\input{\paperroot/discussion}
\input{\paperroot/conclusion}

%\input{doctorat/document/paper-linear-classifier-probes/introduction}
%\input{doctorat/document/paper-linear-classifier-probes/relatedwork}
%\input{doctorat/document/paper-linear-classifier-probes/probes}
%\input{doctorat/document/paper-linear-classifier-probes/experiments}
%\input{doctorat/document/paper-linear-classifier-probes/discussion}
%\input{doctorat/document/paper-linear-classifier-probes/conclusion}

%\chapter{Appendix : Linear Classifier Probes}
%\label{app:paper-linear-classifier-probes}
\begin{subappendices}
    \setcounter{theorem}{0}
    \input{\paperroot/appendix}
\end{subappendices}


==> prologue-linear-classifier-probes.tex <==

\chapter{Prologue to fourth paper : Understanding intermediate layers using linear classifier probes}
\label{chap:prologue-linear-classifier-probes}


\section{Article Details}

\textbf{Understanding intermediate layers using linear classifier probes},
by Guillaume Alain and Yoshua Bengio,
in \textit{International Conference on Learning Representation (2017) (Workshop)}.
%Journal article currently under review in \textit{IEEE Transactions on Neural Networks}.

\textit{Personal Contribution.} This work was all done by me. Naturally, it goes without saying that other people were involved in fruitful discussions about this topic, as always.

\section{Context}

This initial research project that led me to the idea of the
\emph{linear classifier probes} was that I wanted to train a hierarchy of
models of increasing complexity, leading all the way to a very deep neural network
that was basically impossible to train using only traditional backpropagation
from the last layer.

Every model in the collection (except the simplest) relied on a support (a simpler network),
much like a plant can rely on a support (a vertical pole) to help it stand up and grow.
See \citet{romero2014fitnets} for a more explicit implementation of the analogy.
This was both an attempt to train a model of ridiculous depth
(two thousand layers, before the publication of ResNet), and to have a way
to grow a model that exhibits a clear hierarchy of structure.

To monitor this operation, I wanted to develop a tool that would allow me
to see how each component was doing. I wanted to be able to visualize how
complex models would flail around unproductively up until the moment where
their support reached a reasonable state of training.
This would set up a kind of chain reaction, like a fuse that burned
from one end to the other, from simpler to more complex models.
This could be visualized easily by plotting how \emph{good} each model was
(in terms of prediction accuracy of the final layer), but it also
made sense in this case to want to include the prediction accuracy of
every internal layer.
%, despite the fact that these layers were not even used directly for that purpose.
Hence the introduction of \emph{linear classifier probes}.

This original idea described above was not published, and the later work by
\citet{larsson2016fractalnet} shows a very similar architecture.
This context is to convey the idea that the original motivation
behind this article on linear classifier probes was about structure and
hierarchy of representations.


% There is a popular belief that neural networks are blackboxes that cannot be understood.
% This is being repeated despite the fact that many researchers are developing
% techniques to poke around neural networks and are trying to infer the role of
% certain layers with clever visualization techniques.
% The experience of developing and debugging
% a neural network also feels a game of inventing a story to justify each decision
% without really being sure that it is indeed what our model is doing.


\section{Contributions}

We introduce the concept of the \emph{linear classifier probe}.
We add a collection of linear classifiers to be trained using the features of
various layers of a model, and make sure that they do not backpropagate into
the original model. While it could generalized, this concept applies only to
classification problems at the moment.

Technically speaking, this gives us a measurement of how well those features
can be used for the original classification problem. Intuitively, however,
this can guide our understanding about the ``quantity of useful information present
in each layer''. We can diagnose certain problems with models by looking at this measurement.

More importantly, we have observed a very interesting phenomenon while training
deep neural networks for image classification by monitoring them with those probes.
We have observed that the layer representations are naturally acting in a ``greedy'' fashion,
such that every subsequent layer tends to be better than its predecessors in
terms of features for linear classification.
While this experiment observation is intuitively plausible, it does run contrary to
the hypothesis that a deep neural network might ``invest'' some layers to refine a
rich representation that pay off only at the last layer of the model
where the softmax classifier is found.


\section{Recent Developments}

This paper was submitted in many different forms over the course of $\sim 2$ years.
It was successfully accepted as a conference workshop twice.
%accepted only at conference workshops, and thus it took many forms
%over the course of $\sim 2$ years.
%At the current time, the last incarnation of it was rejected by the \textit{IEEE Transactions on Neural Networks} journal.
One of the consequences of this delay is that the idea of linear classifier probes
made its way elsewhere, and there is now a very impressive paper by colleagues
at Google Brain \citep{raghu2017svcca} where a similar idea is presented.
Their particular tool is more general and even more insightful
(albeit more complex and costly) than my own take on linear classifier probes.


%

